Adaptive Stochastic Nonlinear Model Predictive Control with Look-ahead Deep Reinforcement Learning for Autonomous Vehicle Motion Control

In this paper, we present a Deep Reinforcement Learning (RL)-driven Adaptive Stochastic Nonlinear Model Predictive Control (SNMPC) to optimize uncertainty handling, constraints robustification, feasibility, and closed-loop performance. To this end, we conceive an RL agent to proactively anticipate upcoming control tasks and to dynamically determine the most suitable combination of key SNMPC parameters - foremost the robustification factor $\kappa$ and the Uncertainty Propagation Horizon (UPH) $T_u$. We analyze the trained RL agent's decision-making process and highlight its ability to learn context-dependent optimal parameters. One key finding is that adapting the constraints robustification factor with the learned policy reduces conservatism and improves closed-loop performance while adapting UPH renders previously infeasible SNMPC problems feasible when faced with severe disturbances. We showcase the enhanced robustness and feasibility of our Adaptive SNMPC (aSNMPC) through the real-time motion control task of an autonomous passenger vehicle to follow an optimal race line when confronted with significant time-variant disturbances. Experimental findings demonstrate that our look-ahead RL-driven aSNMPC outperforms its Static SNMPC (sSNMPC) counterpart in minimizing the lateral deviation both with accurate and inaccurate disturbance assumptions and even when driving in previously unexplored environments.

==> sections/nominal_nmpc.tex <==
% \todo[inline]{for ACC/ECC keep NMPC and SNMPC more general and then apply it to the trajectory following use-case}
% We use the following Notation. Take a variable $z \in \mathbb{R}$, then $\boldsymbol{z} = [z_0,...,z_n]^T \in \mathbb{R}^n$ is the vector composed of $z$ variables and $\boldsymbol{Z} = [\boldsymbol{z}^{(0)},..., \boldsymbol{z}^{(m)}] \in \mathbb{R}^n \times \mathbb{R}^m$ denotes the matrix of the concatenated vectors $\boldsymbol{z}$.
% We present the nominal NMPC problem that we consider in our work in Problem (\ref{eq:nominal NMPC problem}).

In this work, we consider the following nominal NMPC: 
% formulated in Problem 1.
% We now introduce the nominal NMPC problem considered in our work, presented in Problem (\ref{eq:nominal NMPC problem}).
% \subsection{NMPC Problem Formulation}
\begin{equation}
\begin{aligned}
& \textbf{Problem 1} && \textbf{Nominal NMPC}\\ 
% &&& \textbf{problem}\\
&  \underset{\boldsymbol{x}(.), \boldsymbol{u}(.)}{\min} & & 
\begin{aligned}
    \int^{T_p}_{\tau=0} & l(\boldsymbol{x}(\tau),\boldsymbol{u}(\tau)) \space  d\tau \\ 
 & + m(\boldsymbol{x}(T_p))
\end{aligned}
  \\ 
& \text{subject to} & & \boldsymbol{x}_{0} \leq \boldsymbol{x}(0) \leq \boldsymbol{x}_{0} \text {, }  \\
% & \text{subject to} & & \text { --- initial state ---} \\
% & & &\underline{x}_{0} \leq J_{\mathrm{bx}, 0} \space x(0) \leq \bar{x}_{0} \text {, } \\
% & & &  \text { --- vehicle dynamics ---} \\
& & & \dot{\boldsymbol{x}}(t) = f(\boldsymbol{x}(t),\boldsymbol{u}(t)) \text {, } & t \in[0, T_p), \\
% & & &  \text { --- path constraints ---} \\
& & & \underline{\boldsymbol{h}} \leq h(\boldsymbol{x}(t), \boldsymbol{u}(t)) \leq \bar{\boldsymbol{h}},& t \in[0, T_p), \\
& & & \underline{\boldsymbol{x}} \leq J_{\mathrm{bx}} \space \boldsymbol{x}(t) \leq \bar{\boldsymbol{x}}, & t \in[0, T_p), \\
& & & \underline{\boldsymbol{u}} \leq J_{\mathrm{bu}} \space \boldsymbol{u}(t)\leq \bar{\boldsymbol{u}}, & t \in[0, T_p), \\
% & & &  \text { --- terminal constraints ---} \\
& & & \underline{\boldsymbol{h}}^{\mathrm{e}} \leq h^{\mathrm{e}}(\boldsymbol{x}(T_p)) \leq \bar{\boldsymbol{h}}^{\mathrm{e}}, \\
& & & \underline{\boldsymbol{x}}^{\mathrm{e}} \leq J_{\mathrm{bx}}^{\mathrm{e}} \space \boldsymbol{x}(T_p) \leq \bar{\boldsymbol{x}}^{\mathrm{e}}, \\
\end{aligned}
\label{eq:nominal NMPC problem}
\end{equation}
% \todo[inline]{describe each line in plain text, add L1 and L2 terms}
Here, $\boldsymbol{x} \in \mathbb{R}^{n_x}$ denotes the state vector, $\boldsymbol{u} \in \mathbb{R}^{n_u}$ the control vector, $t$ the discrete time, $T_p$ the prediction horizon, $f$ the system dynamics, $h$ and $h_e$ the path and terminal nonlinear inequality constraints, $J_{bx}$ and $J_{bx}^e$ help express linear path and terminal state constraints, $J_{bu}$ helps express control input constraints and $x_0$ the initial state.
% \subsection{Cost Function}
Also, $l: \mathbb{R}^{n_{\mathrm{x}}} \times \mathbb{R}^{n_{\mathrm{u}}}  \rightarrow \mathbb{R}$ denotes the stage cost and $m: \mathbb{R}^{n_{\mathrm{x}}}  \rightarrow \mathbb{R}$ the terminal cost.

==> sections/related_work.tex <==
% keep it short only about SNMPC:
% start with 2012 (Fagiano) \cite{fagiano2012nonlinear}, 2014 (Mesbah) \cite{mesbah2014stochastic}, 2014 (Streif) 
% go on the difference and the evolotution between the different papers then introduce the evolution/upgrade we do in this paper. 


% - Dealing with disturbances
% - Dealing with disturbances in NMPC
% - Robust NMPC
% - Stochastic Linear MPC
% - Stochastic NMPC
% - Motion control application (disturbances + NMPC / disturbances + MPC)
% \cite{falcone2007linear} 

% The rest of the paper is structured as follows. In Sec.\ref{sec:nominal_nmpc}, ... 

Stochastic uncertainties are nonnegligible in complex dynamic system and can cause unpredicted and undesired system output if a nominal NMPC is used, hence lead a bad closed-loop performance. To handle these uncertainties, two variant of NMPC, namely Robust NMPC and stochatic NMPC can be applied.

Robust NMPC assumes bounded uncertainties and enables analyzing the stability and performance of the system against worst-case perturbations. This has led to a number of applications, where providing guarantees on robust stability and performance is the main objective [1], [2]. However, the worst-case perturbations may have a extremely small probability of occurrence in real practice [3], so control design based on worst-case uncertainties can be too conservative and, therefore, may lead to infeasible control problems. In addition, it is seldom practical to specify precisely the uncertainty bounds.

In contrast, SNMPC with chance constraints adopts a distinctive strategy to solve MPC problems under uncertainties. It ultilizes probabilistic descriptions of uncertainties and constraint violations, allowing for acceptable levels of risk during system operation. Chance constraints offers the possibility to trade off between closed-loop performance and constraints violation, which mitigate the inherent conservativeness in robust NMPC.

Unlike linear SMPC, SNMPC has been much less developed due to the difficulty in efficient UP through nonlinear system. SNMPC can be broadly categotized in terms of the underlying UP method. The use of Markov-chain Monte Carlo \cite{maciejowski2007nmpc} techniques was initially proposed that didn't rely on convexity assumptions and guaranteed convergence to near-optimal solutions under certain conditions related to the convergence of a homogeneous Markov chain. However, their effectiveness when implemented in a receding-horizon manner remained unproven. Sequential Monte Carlo was adopted in \cite{kantas2009sequential} to further improve effectiveness.

To deal with the difficulties of efficient UP, Gaussian-mixture approximation method \cite{weissel2009stochastic} was used to describe the transition probability distributions of states. This approach allowed for a flexible framework for constructing the probability distributions of stochastic variables, enabling a more comprehensive representation of uncertainty.

The gPC approach \cite{fagiano2012nonlinear} \cite{mesbah2014stochastic} was afterwards proposed to address time-invariant stochastic uncertainties in both system parameters and initial conditions. The gPC framework replaces the conventional implicit mappings between uncertain variables/parameters and states, providing an efficient method for predicting the time evolution of the moments of probability distributions of stochastic states.

All works using gPC framework aims to control a system in a relative stable environment with a fixed control objective under uncertainty. In this work, we further extend this framework to a motion control application with a novel UPH concept, which helps stabilizing SNMPC during UP. This application aims to make a vehicle with highly nonlinear dynamics track a time-varying reference trajectory, which means both external environent and control objective vary frequently over time.

The rest of paper is structured as follows. In \ref{sec:nominal_nmpc}, the nominal NMPC problem will be formulated. Afterwards, \ref{sec:stochastic_nmpc} introduces the implementations and novelty of this paper. In \ref{sec:traj_following} the formulation of trajectory following application will be presented and the simulation results will be discussed in \ref{sec:sim_results}. At last, we will conclude the results and give a outlook for further research.
